VerdictDB: Universalizing Approximate Query Processing

Despite 25 years of research in academia, approximate query processing (AQP) has had little industrial adoption. One of the major causes of this slow adoption is the reluctance of traditional vendors to make radical changes to their legacy codebases, and the preoccupation of newer vendors (e.g., SQL-on-Hadoop products) with implementing standard features. Additionally, the few AQP engines that are available are each tied to a specific platform and require users to completely abandon their existing databases---an unrealistic expectation given the infancy of the AQP technology. Therefore, we argue that a universal solution is needed: a database-agnostic approximation engine that will widen the reach of this emerging technology across various platforms. Our proposal, called VerdictDB, uses a middleware architecture that requires no changes to the backend database, and thus, can work with all off-the-shelf engines. Operating at the driver-level, VerdictDB intercepts analytical queries issued to the database and rewrites them into another query that, if executed by any standard relational engine, will yield sufficient information for computing an approximate answer. VerdictDB uses the returned result set to compute an approximate answer and error estimates, which are then passed on to the user or application. However, lack of access to the query execution layer introduces significant challenges in terms of generality, correctness, and efficiency. This paper shows how VerdictDB overcomes these challenges and delivers up to 171$\times$ speedup (18.45$\times$ on average) for a variety of existing engines, such as Impala, Spark SQL, and Amazon Redshift, while incurring less than 2.6% relative error. VerdictDB is open-sourced under Apache License.

==> figures/join_rules.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l l l l l l}
\hline
           & \textbf{nosample} & \textbf{uniform} & \textbf{hashing} & \textbf{stratified} & \textbf{irregular} \\ \hline
\textbf{nosample}   & nosample & uniform  & hashing     & stratified & irregular \\
\textbf{uniform}    & $\cdot$  & uniform  & irregular   & irregular  & irregular \\
\textbf{hashing}    & $\cdot$  & $\cdot$  & hashing$^*$ & irregular  & irregular \\
\textbf{stratified} & $\cdot$  & $\cdot$  & $\cdot$     & stratified$^*$ & irregular   \\
\textbf{universe}   & $\cdot$  & $\cdot$  & $\cdot$     & $\cdot$    & irregular \\
\hline
\end{tabular}
\vspace{2mm}
\caption{Join rules for sample tables. * requires that the sample tables were built on the same column set.
% Joining the sample tables in the column and row headings produces a sample table whose type is as specified in the cells. * requires that the stratified samples (or universe samples) to be joined are built on the same column set.
}
\label{tab:join_rules}
\end{table}

==> ola.tex <==
%!TEX root = verdict.tex

\section{Applying Variational Subsampling to Online Aggregation}
\label{sec:ola}

\input{figures/exp_ola}

\tofix{Our proposed error estimation technique (i.e., variational subsampling) can also 
	be used to support latency bounds for important classes of queries (i.e., those without aggregations of aggregations) by performing online aggregation. Specifically, we can continuously refine and report the current error estimates, hence allowing the application to stop the query execution as soon as a specific  time period has elapsed.
To support online aggregation, we must compute error bounds in an incremental fashion without re-aggregating the tuples that have been aggregated before.}

\tofix{
The approach of variational subsampling is amenable to such incremental aggregation. Recall that variational subsampling relies on variational tables, which are created by assigning random integers to sampled tuples. 
Therefore, when processing a new set of tuples in online aggregation, 
we can  construct the variational tables in an incremental fashion by assigning a new set of random integers to the new set of tuples. The only difference is that we must also increase the total number of subsamples conceptually (since we have assigned a new set of integers).}

\tofix{
To demonstrate that variational subsampling can be easily modified to support online aggregation, we have implemented a prototype
of this idea, and have performed additional experiments. Our prototype performs ripple join, exploiting the partitioning features supported by 
most modern query engines (e.g., Hive, Impala, Spark). When a table is partitioned on a certain column (e.g., \texttt{part\_num}), one can efficiently access the tuples associated with a certain value in the partitioning column (i.e., \texttt{part\_num} = 1). Our prototype retrieves
	 joined tuples in an incremental fashion (by ripple join) using randomly-generated partition numbers. The rewritten queries include the error estimation logic of variational subsampling.}

\tofix{
We compared this prototype against another online aggregation engine, XDB~\cite{wander-join}, which that relies on a state-of-the-art join algorithm. 
Since XDB's join algorithm requires B-trees, their engine is tightly integrated into a traditional database, PostgreSQL. 
Here, we used the same benchmark queries used in~\cite{wander-join}.
\cref{exp:ola} shows the results.
In general, our prototype produced more accurate answers given the same time bound.
% One can observe that, our prototype system employing variational subsampling produced more accurate answers, in general.
This was mainly due to the fact that our middleware-based query rewriting technique enabled us to use the distributed computational power 
of Impala. In contrast, XDB had to run on a single machine due to its close integration with PostgreSQL; thus, its scalability was relatively limited. 
% <<<<<<< HEAD
% If a distributed version of XDB's join algorithm was  available, we would expect it to achieve a better performance than \verdict, 
% 	due to its tight integration.
% =======
If a distributed version of XDB's join algorithm was  available, we would expect it to achieve a better performance than our middleware,
	simply due to its tight integration with the database.
% >>>>>>> 4e3a8faeb2e78c51e14755379f9a1176ed4c44d4
 However, its tight integration still limits its applicability to a certain target database system.
}


==> other_aggregates.tex <==
\section{Other Aggregates}
\label{sec:other_aggregates}

\section{Cases for Nested Variational Table}
\label{sec:nested_var}

% \yongjoo{The section title must change.}

\ph{Case 1 (hashed sample):}
If the following two conditions---(1) the \texttt{orders\_subsample} table is a hashed sample with a sampling parameter $\tau$, and (2) \tofix{the column on the hashed sample is built on is identical to the grouping attributes}, then \texttt{t\_subsample} is a uniform sample of \texttt{t} with a sampling parameter $\tau$. This is because only a subset of the groups in the \texttt{group-by} result will be present, and its probability is exactly $\tau$.

\ph{Case 2 (stratified sample):}
If the \texttt{orders\_subsample} is a \{stratified sample with a sampling parameter $\tau$,  \tofix{and the column on the stratified sample is built on is identical to the grouping attributes}, then \texttt{t\_subsample} is a simple random sample of \texttt{t} with a sampling parameter 1. This is because no groups will be missed.

==> query_latencies.tex <==
\section{Raw Query Latencies}
\label{sec:query_latencies}



==> query_specification.tex <==
\section{Query Specification}
\label{sec:query_specification}

\begin{table}[H]
\begin{tabular}{l l l}
\Xhline{2\arrayrulewidth}
Name & Characteristics \\ \hline
t1   & A single fact table \\
t9   & Contains a subquery with joins of 6 tables \\
t12  & A join of two tables; \texttt{case} in aggregate functions \\
t15  & High cardinality attribute in \texttt{group-by} \\
t17  & Comparison to a subquery expression \\
c1   & A single fact table \\
c2   & A join of three tables \\
c3   & A join of four tables \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Queries used in our experiments and their properties. Experiment results with more queries are provided in our extended report~\cite{extendedreport}.}
\label{tab:exp:queries}
\end{table}

==> real-world.tex <==
%!TEX root = verdict.tex

\section{Real-world Use-cases}
\label{sec:usecases}

\newcommand{\walmart}{\textsc{Company1}\xspace} % walmart
\newcommand{\dunnhumby}{\textsc{Company2}\xspace} % dunnhumby
\newcommand{\thescore}{\textsc{Company3}\xspace} % thescore

Despite being in its early stages of adoption,
	\verdict has already found a few early users.
In this section, we briefly share the use-cases 
	that \verdict has been deployed for in these companies,
		which we anonymously refer to as \walmart, \dunnhumby, and \thescore.
None of these companies has had to modify their existing applications:
(1) they all connect 
to \verdict (and the underlying database) either using JDBC drivers or by including \verdict's jar file in Spark's --jar option, and
(2) \verdict's output is consistent with existing connections methods (i.e., java.sql.ResultSet for JDBC and spark.sql.DataFrame for Spark).

%We closely worked with three international companies that performed large-scale data analytics. We refer to those companies as \walmart, \dunnhumby, and \thescore.
 % \coma and \comb were customer science companies, and \comc was a digital media company.

% multinational retailing corporation retailing corporation chain of hypermarkets, discount department stores, and grocery stores

% theScore creates mobile-first sports experiences, connecting fans to what they love through an addictive combination of real-time news, scores, fantasy information and alerts while creating and curating content that is mobile optimized, comprehensive, customizable and seamlessly shareable.

% Dunnhumby is a UK-based customer science company
% From effective prices and promotions and better ranging & assortment, to personalised and relevant customer communication plans and advertising. Which ever the need, we partner with you to help transform your business.

As a  multinational retailing corporation, \walmart's marketing department analyzes collected transaction data to identify customer demographics who would most positively respond to its email marketing. Each day, 400 GB worth of data (370M rows and 91 columns) are ingested into a Hive table (append-only),
	which are then queried using \walmart's on-premise Hive and Spark clusters.
Their most common type of query  
	are \texttt{count(*)} queries with various selection predicates. 
\walmart uses \verdict to speed up these queries, which would previously take 20+ minutes.



\dunnhumby is a customer science company, collecting and analyzing data on behalf of major corporations
	to help them with better pricing, promotions, personalized communications, and targeted ads.
Its data is ingested into an HDFS cluster, and 
%	\tofix{a typical dataset has over 300M transactions from 500 thousand distinct customers.}\barzan{makes no sense! each customer made 1M transactions almost?} 
(after ETL) analyzed on-premise, using SQL (Hive and Spark)  and Python.
	 %however, it was also considering to migrate to Google Dataproc. \dunnhumby used both SQL and Python for its data analytics.
Most of its analysts collect basic statistics, while a few data scientists also train and use machine learning models. % random forests
\dunnhumby is using \verdict for speeding up the first category (e.g., total sales by brand over a join in a star schema).
	
\thescore is a digital media company. It ingests streaming (sports) data in a semi-batch mode into Amazon Redshift (40 tables).
% with 20--100 data analysts. \thescore ingested stream data in a semi-batch mode into RedShift. Here, semi-batch mode means that data was collected for a short period of time and those collected data was ingested into RedShift.
%\thescore has about 12TB of data in RedShift. %Among them, 1--2TB of data (40 tables) could be analyzed at any time.
The dataset (12TB) is queried by 100+ data analysts, via a variety of interfaces (PostreSQL, Navicat, SQLAlchemy, Periscope Data).
Instead of reducing latency, 
	\thescore's main reason for using \verdict is to reduce load on its operational cluster;
\verdict operates on a separate, smaller cluster with 1--2TB of data, and is queried by about 20 analysts.


\ignore{
Two of the three companies were using open-source database systems; however, none of those companies deployed the database systems by themselves. That is, \coma and \comb were using the database systems shipped in pre-packaged solutions (i.e., Cloudera and MapR); \comc was using a database system available via cloud (i.e., Amazon Redshift). For this reason, making modifications to any of those database systems was hardly possible.

They had ETL (Extract-Transform-Load) pipelines that periodically ingested data into schema-based database systems by which SQL was supported. In some cases, not all data analytics were familiar with SQL. \comc had front-end applications that provided visualizations (e.g., Tableau, Periscope Data). \comb used Jupyter notebook; \comb was even investing in developing a natural-language interface that would translate English sentences into SQL statements. However, in most cases, SQL was still central to their daily data analytics.

All three companies showed interests in using \verdict due to the long latencies of their queries. 
Although the sizes of the data for which they wanted interactive analytics varied (40 GB--2 TB),
their query latencies were typically longer than 10 minutes. We believe it was partly due to the differences in the size of their clusters and the actual amount of resources allocated per data analyst. For instance, \comb mentioned it was not considering Impala in its production environment due to the lack of support of Yarn.\footnote{At time of writing, Impala started to support Yarn in its non-production version.} This also implies that not all three companies were spending enough budget to reduce query latencies below 10 seconds, solely relying on horizontal scaling.

\verdict started to support various interfaces, such as the Kerberos authentication, metadata schema configurations, Jupyter notebooks, etc., due to those companies' requests. Currently, they either connect to \verdict (and to the underlying database) either using JDBC drivers or by including \verdict's jar file in Spark's `--jar' option. Since \verdict operates at the driver level, the engineers and data analysts at those companies could use \verdict without touching either on-premise clusters or cloud systems. The output from \verdict was consistent with existing connections methods, i.e., \texttt{java.sql.ResultSet} for JDBC and \texttt{spark.sql.DataFrame} for Spark; thus, front-end applications (e.g., Apache Hue, Apache Zeppelin) could consume the results from \verdict seamlessly.
}

% \barzan{Write a short paragraph explaining how each of Walmart Labs, Dunnhumby and theScore are or plan to use Verdict. Explain their 
% usecase and replace their names with a description of what they do and why and how they use Verdict. Also, mention what DB they currently use}

% \barzan{I am debating where to put this section: putting it right before expr is a bit out of place. Putting it in sec 2 as a subsection is a good idea but 
% sec 2 is already too long. Moving it to right before conclusion is yet another option}
